MTrainS: Improving DLRM training efficiency using heterogeneous memories

Recommendation models are very large, requiring terabytes (TB) of memory during training. In pursuit of better quality, the model size and complexity grow over time, which requires additional training data to avoid overfitting. This model growth demands a large number of resources in data centers. Hence, training efficiency is becoming considerably more important to keep the data center power demand manageable. In Deep Learning Recommendation Models (DLRM), sparse features capturing categorical inputs through embedding tables are the major contributors to model size and require high memory bandwidth. In this paper, we study the bandwidth requirement and locality of embedding tables in real-world deployed models. We observe that the bandwidth requirement is not uniform across different tables and that embedding tables show high temporal locality. We then design MTrainS, which leverages heterogeneous memory, including byte and block addressable Storage Class Memory for DLRM hierarchically. MTrainS allows for higher memory capacity per node and increases training efficiency by lowering the need to scale out to multiple hosts in memory capacity bound use cases. By optimizing the platform memory hierarchy, we reduce the number of nodes for training by 4-8X, saving power and cost of training while meeting our target training performance.

==> Discussion_and_future_works.tex <==
%%\vspace{-3mm}
\section{Discussion and future work}\label{discussion}
%%\vspace{-3mm}

In this paper, we demonstrate that using different storage class memories helps us reduce the number of nodes used for training by 4-8$\times$ for capacity-bound DLRM models. We learned that for models that are both capacity and bandwidth bound, the additional memory bandwidth with storage class memories is not enough to accommodate the models. Our results show that while we can use \pmem~with \flash~ to meet our QPS target, server configuration with just \optane~ can meet our target QPS for current models. For future scaling using \pmem~ and \optane~ can help us meet our target QPS. Although these memories are slower than DRAM, they provide enough performance for our memory capacity-bound workloads. Hence we can harness the cost and power benefit of SCMs. In the future, we plan to extend our systems with Compute Express Link (CXL) to access \pmem, which will provide us with better memory bandwidth because we don't have to share the memory bus with DRAM and we wont be limited by the system's available DIMM slots. This will help our design to suit bandwidth-bound workloads too. 

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> ev2.tex <==
%\vspace{-3mm}
\section{Evaluation}\label{experiments}
\subsection{Baseline}
We compare \ourway~ to the baseline system configuration shown in Table \ref{tab:systems}. Our implementation in the baseline also uses an integration of DLRM and FBGEMM\_GPU. We use HBM and DRAM in the baseline for embedding storage and caching. This implementation uses the same techniques as CDLRM \cite{balasubramanian2021cdlrm}. While CDLRM uses the CPU to manage the cache, for a fair comparison with \ourway, which uses GPU for fast cache management, we move the cache management in CDLRM to GPU. We call this CDLRM+. We also added the efficient embedding table placement in CDLRM+. Our experiments compare the number of nodes required to train a model running CDLRM+ with the performance we get with a single node running \ourway. To compare performance, we use target QPS, an acceptable QPS in our data center, to train a specific model based on how often we need to train models and the rate at which new training data becomes available. QPS in our experiment represents the number of input data we can use to train a model per second, including the forward and backward pass. It is inversely proportional to the training time.   

\vspace{-1mm}
\subsection{Training efficiency}
One of the principal arguments for adopting denser memory technologies is to use fewer nodes for specific model training and improve power and cost-efficiency. Hence, we first compare the overall deployment efficiency of \ourway~and CDLRM+ for \ifrmodel~and \adsmodel~ based on the target QPS and the power and energy.
\begin{figure}[]
%%\vspace{-3mm}
\vspace{-10mm}

 \centering
 \includegraphics[width=0.43\textwidth, trim={0.25cm 6.8cm 5.3cm 0.05cm },clip]{Figures/qps_target_1.pdf}
 %\vspace{-2mm}
 \caption{\footnotesize{ Training QPS and number of host Comparison of CDLRM+ and \ourway~ with SLA QPS target as the baseline for \ifrmodel~ and \ifrmodelscaled }}
 \label{scale_model_1}
 \vspace{-3mm}
\end{figure}
\begin{figure}[]
%\vspace{-10mm}

 \centering
\includegraphics[width=0.44\textwidth, trim={0.25cm 7.1cm 5.3cm 0.05cm },clip]{Figures/qps_target_ads_1.pdf} 
 \caption{\footnotesize{ Training QPS and number of host Comparison of CDLRM+ and \ourway~ with SLA QPS target as the baseline for \adsmodel.}}
\vspace{-4mm}
 \label{scale_model_2}
\end{figure}
%\vspace{-1mm}
\subsubsection{\textbf{Deployment efficiency}}

Figure \ref{scale_model_1} shows the efficiency comparison of \ifrmodel~and \ifrmodelscaled, which are memory capacity bound. Note that \ifrmodelscaled~ is the future scaling of \ifrmodel~ with a larger size (2$\times$). These models require 4-8 hosts to load and train with the baseline CDLRM+. With \ourway, one host can provide sufficient extended memory capacity to load and train the model. We can also reach the target QPS (SLA) in such a setting, as seen in Figure \ref{scale_model_1}. While the baseline without \ourway~ achieves higher QPS, it requires 4-8$\times$ more hosts, so this performance is stranded and does not contribute additional efficiency to the deployment because we already met our training QPS requirement. As a result, \ourway~ can improve power and cost efficiency for \ifrmodel~ and \ifrmodelscaled~ while providing SLA performance. Our experiments show that models scaled beyond \ifrmodelscaled require multi-node training, each node leveraging \ourway. Nevertheless, \ourway~ still provides a lower host count because it can store a larger model per host compared to the baseline.  

Figure \ref{scale_model_2} shows a comparison of \ourway~vs CDLRM+ for \adsmodel~ ( BW bound workload). This model requires 3 hosts to load and train with the baseline configuration using CDLRM+. While \ourway~allows the model to be loaded and trained on one host, it does not meet the QPS requirements because of the higher memory bandwidth required by the model. Also shown in the figure, using 2 nodes, each running \ourway, significantly improves performance compared to the single node. However, the 2 nodes still fail to meet the QPS target because the additional BW with SCMs in the system, even with 2 nodes, is not enough to accommodate the high BW demand of \adsmodel. However, such capability extends the efficiency of research and development without high QPS production requirements.

%In contrast, X and Y nodes are required to load the model with \pmem~or \flash~ respectively. Figure~\ref{fig:qps_ifr} shows the training QPS with different optimization and configurations. The first observation is that leveraging \optane can increase QPS by up to Z\% compared to \flash, given the lower latency and higher IOPS offered by \optane. \pmem can further increase QPS, by up to 90\% compared to \flash, by allowing bigger cache for the SSDs. 

%Given the QPS with HBM and DRAM only solution, QPS per host could be improved by G\% by avoiding the scale out. 

%We need cache hit rates, and SSD IOPS, and also discuss how much of SSD BW we are actually consuming. 
%We might need a model with a few more large features to increase BW to SSD.
%As seen in Figure \ref{scale_model_1} when we add \pmem to SSD training we achieve 1.6 - 1.85X more QPS for \ifrmodel. We can conclude that the increase in performance is due to the addition of \pmem which will increase the cache hit rate. Even when we are increasing the size of the model by 2-4X we can still accommodate for the increase in size and BW requirement. This is because of the high locality of the embedding features and with hierarchical caching, we can keep the highly accessed data in DRAM, which will provide high BW to the hot data. 




\vspace{-1mm}
\subsubsection{\textbf{Power and energy analysis}}
%%\vspace{-3mm}

 
Figure \ref{fig:baseline_energy} shows the power and energy of \ifrmodel~ and \ifrmodelscaled~  using \ourway compared to the baseline configuration with only HBM and DRAM. Compared to training using the baseline, which requires 4-8 nodes to accommodate the models, we see $\sim$ 1/4 - 1/8  power reduction with \ourway. This reduction is mainly driven by the decrease in the number of nodes required for training with 
\ourway. This leads to up to 50\% energy reduction. However, as seen in the figure, \sysOne has higher energy than the baseline system because of the low QPS (longer training time). Note that this high reduction is because we have a QPS target for training. If we were to compare absolute performance achieved by the baseline system and \ourway, the number of nodes running \ourway required would be higher, lowering power and energy reduction.

%Figure R\ref{fig:adsbaseline_energy} shows the power and energy comparison of the baseline system with various MTrainS configurations. In the figure, we see that the average power consumption is reduced by up to 60\%  in 1 node and 30\% in 2 node MTrainS for the configurations with SCM (reduction is because of the number of nodes used compared to baseline). But when we see energy, as seen in figure 13 in the paper, the QPS for model 2 for SCM and NAND SSD training is low compared to baseline config (higher training time), hence energy consumption is very high compared to the baseline. This shows that, for bandwidth-bound workload, using storage class memories does not meet the QPS target and increases energy consumption.

%Figure \ref{fig:adsbaseline_energy} shows \adsmodel's average power consumption is reduced by up to 60\% in 1 node and 30\% in 2 node \ourway configurations. Nonetheless, when we see energy in Figure \ref{fig:adsbaseline_energy} because \ourway's QPS for model 2 is significantly lower than the baseline config (longer training time), energy consumption is higher compared to the baseline in all configurations. In summary, for bandwidth-bound workload, using \ourway does not meet the QPS target and increases energy consumption.
Figure \ref{fig:adsbaseline_energy} shows \adsmodel's average power consumption is reduced by up to 60\% in 1 node and 30\% in 2 node \ourway configurations. Nonetheless, because \ourway's QPS for  \adsmodel is considerably lower than the baseline config (longer training time), even when using 2 nodes running \ourway, energy consumption is higher compared to the baseline in all configurations, as seen in Figure \ref{fig:adsbaseline_energy}. In summary, for bandwidth-bound workload, using \ourway does not meet the QPS target and increases energy consumption.

\begin{figure}[]
\vspace{-10mm}
 \centering
  \includegraphics[width=0.450\textwidth, trim={0.2cm 10.0cm 10.3cm 0.05cm },clip]{Figures/power_e_baseline.pdf}
   \vspace{-3mm}

 \caption{\footnotesize{Power and energy comparison of \ourway~ to baseline system running CLDRM+ for \ifrmodel~ and \ifrmodelscaled .}}
 \vspace{-6mm}
 \label{fig:baseline_energy}
\end{figure}
\begin{figure}[]
%\vspace{-9mm}
 \centering
  \includegraphics[width=0.450\textwidth, trim={0.2cm 9.5cm 11.3cm 0.05cm },clip]{Figures/model2_power.pdf}
  % \vspace{-3mm}

 \caption{\footnotesize{Power and energy comparison of \ourway~ to baseline system running CLDRM+ for \adsmodel~ using 1 and 2 nodes eith MTrainS.}}
 \vspace{-3mm}
 \label{fig:adsbaseline_energy}
\end{figure}

\subsection{MtrainS configs performance, energy, and power differences}

Next, we evaluate the performance of the various \MTrainS system configurations compared to \sysOne~ to understand the performance implication of \pmem~ and \optane~ compared to \flash. In Figure \ref{fig:qps_ifr} and \ref{fig:qps_ifr_scaled}, we compare QPS achieved for \ifrmodel~ and \ifrmodelscaled~ for different configurations of \ourway. As shown in Figure \ref{fig:qps_ifr}, for \ifrmodel, using \optane~(\sysTwo) instead of \flash~(\sysOne) increases QPS by 2$\times$. Using \pmem~with \flash~(\sysThree~ and \sysFour) increases cache size. Hence lowers traffic to \flash~ and therefore provides 2.4$\times$ QPS. Our results indicate no further improvement in QPS for the setup with both \pmem~and \optane~ for \sysFive because once we increase the cache size per host using \pmem, the access to SSDs is out of the critical path. 


%(training with \flash~ without SCM).



%For 2X size \ifrmodel, as seen in Figure \ref{fig:qps_ads}, using \flash~ with 384GB of \pmem~ increases QPS by 1.73X whereas, using 768GB of \pmem increases by 2.76X due to the increased cache hit rate. When we compare using both \pmem~ with \flash, we achieve 3.2X QPS. 2X model has much higher IO traffic than \ifrmodel~ . In this case even after we increased the cache size with \pmem~, using \optane still provides better performance because the SSD access, even though decreases using \pmem~ cache, is still in the critical path. 
\begin{figure}[t!]
%\centering
\vspace{-10mm}

  \begin{subfigure}{.50\columnwidth}

%\includegraphics[width=1.16\textwidth, trim={0.01cm 8.5cm 16.9cm 0.05cm },clip]{Figures/feed_qps_1x_1.pdf}
\includegraphics[width=1.16\textwidth, trim={0.6cm 11.5cm 16.9cm 0.05cm },clip]{Figures/model1_detail.pdf}
%%%\vspace{-3mm}
%\vspace{-5mm}
\caption{\textmd{\ifrmodel} }
%%%\vspace{-3mm}
\label{fig:qps_ifr}
    \end{subfigure}
\begin{subfigure}{0.46\columnwidth}
%\centering
%\includegraphics[width=1.15\textwidth, trim={0.05cm 8.0cm 17.02cm 0.05cm },clip]{Figures/feed_qps_2x_1.pdf}
\includegraphics[width=1.14\textwidth, trim={0.1cm 11.5cm 18.9cm 0.05cm },clip]{Figures/model1p_detail.pdf}

%%%\vspace{-3mm}
%\vspace{-5mm}
\caption{\textmd{\ifrmodelscaled}}
%%%\vspace{-3mm}
\label{fig:qps_ifr_scaled}

    \end{subfigure}
 \caption{\footnotesize{QPS comparison of different configuration of \ourway~ with \sysOne as the baseline for \ifrmodel and \ifrmodelscaled.}}
\vspace{-3mm}
%\label{figures:cache_hit}
\end{figure}



\begin{figure}[t!]
%\centering
%\vspace{-8mm}

  \begin{subfigure}{.50\columnwidth}

%\includegraphics[width=1.16\textwidth, trim={0.01cm 8.5cm 16.9cm 0.05cm },clip]{Figures/feed_qps_1x_1.pdf}
\includegraphics[width=1.21\textwidth, trim={0.5cm 11.5cm 16.5cm 0.05cm },clip]{Figures/model2_1_detail.pdf}
%%%\vspace{-3mm}
%\vspace{-5mm}
\caption{\textmd{1 Node \ourway} }
%%%\vspace{-3mm}
\label{fig:qps_ads}
    \end{subfigure}
\begin{subfigure}{0.46\columnwidth}
%\centering
%\includegraphics[width=1.15\textwidth, trim={0.05cm 8.0cm 17.02cm 0.05cm },clip]{Figures/feed_qps_2x_1.pdf}
\includegraphics[width=1.14\textwidth, trim={0.1cm 11.7cm 19.09cm 0.05cm },clip]{Figures/model2_2_detail.pdf}

%%%\vspace{-3mm}
%\vspace{-5mm}
\caption{\textmd{2 Nodes \ourway}}
%%%\vspace{-3mm}
\label{fig:qps_ads_2}

    \end{subfigure}
 \caption{\footnotesize{QPS comparison of different configuration of \ourway~ with \sysOne as the baseline for \adsmodel.}}
\vspace{-6mm}
%\label{figures:cache_hit}
\end{figure}

For \ifrmodelscaled, shown in Figure \ref{fig:qps_ifr_scaled}, \flash~with 384GB of \pmem~(\sysThree) increases QPS by 1.73$\times$ whereas, 768GB of \pmem~(\sysFour) increases by 2.76$\times$ due to the increased cache hit rate. When we use both \pmem~with \optane~(\sysFive), we achieve 3$\times$ QPS. \ifrmodelscaled~has higher BW requirement due to increased embedding dimension. With \flash~we already read 4KB blocks per IO, which is larger than the embedding dimension. Nevertheless, increased embedding dimension results in fewer embedding rows maintained in the cache (DRAM or \pmem), given fixed cache size. This increases the miss rate and hence results in increased IO to the SSDs. \optane~with higher IOPS can support such an increase in IO, hence showing higher QPS. 

In Figure \ref{fig:qps_ads} for \adsmodel with 1 node \ourway, because of \optane's higher bandwidth and lower latency compared to \flash in \sysOne, performance increases by ~2.2x. By adding \pmem we get 2x and 3.2x more performance because the cache hit increases. Similar to \ifrmodel, the combination of \pmem and \optane achieves the best performance. In figure \ref{fig:qps_ads_2}, the model is sharded between 2 nodes, and the model size per node is half of 1 node \ourway. The performance improvement for 2 nodes follows the same pattern as 1 node \ourway, but the speedup decreases compared to 1 node because SSD traffic decreases when the model size per node is reduced. Although compared to \sysOne, the various configurations show performance improvement for \adsmodel, using SCM does not provide adequate performance (QPS improvement) for memory bandwidth-bound workloads.


In Figure ~\ref{figures:power_1x} and Figure~\ref{figures:power_2x} we show the power and energy of the various \ourway~ configurations \ifrmodel~ and \ifrmodelscaled~ to study the increase in power and the total energy usage when introducing \pmem~ and \optane to our system. 
The power consumption of adding \pmem~ and \optane~ only increases the overall platform power consumption by 1-3.2\%. This is because of the low power consumption of these individual units and because major power consumption contributors are the GPU, CPU, and DRAM. This extra power consumption per node is justified when considering reduced execution time and overall Energy consumption ($Energy = Power \times Time$). We observe a 60\% to 70\% reduction in the energy consumption across the two models compared to \sysOne. Figure \ref{figures:power_ads} and \ref{figures:power_ads_2} show the power and energy of \ourway~ for \adsmodel. In this case, adding SCMs increases the power by 18\%. This is because there are more cache and embedding storage activities in \adsmodel because it has a larger data access volume compared to \ifrmodel.





%%\vspace{-4mm}
 


% Reducing the number of hosts by 4-8 decreases training costs by approximately 4-8. To compare the implication of adding SCM, we compared the additional cost of memory in the system when introducing SCM and with equal addition of DRAM. Due to the limited DRAM in our system, we scaled down the workload size and system configuration to mimic the system with larger DRAM. Table \ref{tab:memorycost} shows a comparison of memory cost and QPS achieved. As seen in the Table, for model 1 while we meet QPS with \systemone, we can meet our endurance with \systemtwo by only adding 0.38% of the cost of total memory. For model 1+, 








%\begin{figure}[]
%\centering
% \includegraphics[width=0.5\textwidth, trim={0.05cm 9.6cm 9.3cm 0.05cm %},clip]{Figures/feed_scale.pdf}
% \caption{SSD training efficiency as we scale models for model 1 .}
% \label{scale_model_1}
%\end{figure}


\subsection{Storage endurance and wear out}
In this and the following sections, we show detailed hardware characteristic analysis of \ifrmodel~ and \ifrmodelscaled because they are the models that benefit from \ourway. Figure \ref{fig:endurance} measures the TB written per day for \ifrmodel~ and \ifrmodelscaled~ to study if we meet our endurance requirements with the diverse configurations of \ourway. Based on the sizes of \optane~ and \flash, the endurances to avoid storage wear out are 200TB and 8TB data writes per day (DWPD), respectively. As seen in the figure, while we satisfy our QPS target with \sysOne~ for \ifrmodel, the write per day exceeds the endurance of \flash~(8TB). \sysThree~ and \sysFour satisfy the endurance because of the increase in cache size that decreases writes to storage. All configurations with \optane (\sysTwo and \sysFive) meet the endurance because of its higher DWPD (200TB). For \ifrmodelscaled, all configurations backed by \flash do not meet the endurance. Therefore, for future models \optane~ is the best option to prevent storage wear out.
\begin{figure}[t!]
\vspace{-10mm}
\begin{subfigure}{.48\columnwidth}
%\includegraphics[width=1.2\textwidth, trim={0.05cm 9.0cm 14.0cm 0.05cm },clip]{Figures/power_m1.pdf}
\includegraphics[width=1.3\textwidth, trim={0.05cm 9.0cm 14.5cm 0.95cm },clip]{Figures/power_pact_m1.pdf}
\vspace{-6mm}
\caption{\textmd{\ifrmodel} }
\vspace{-1mm}
\label{figures:power_1x}
    \end{subfigure}
\begin{subfigure}{0.48\columnwidth}
%\centering
%\includegraphics[width=1.0\textwidth, trim={0.05cm 8.8cm 17.5cm 0.08cm },clip]{Figures/power_m1p.pdf}
\includegraphics[width=1.0\textwidth, trim={0.05cm 8.6cm 18.9cm 0.95cm },clip]{Figures/power_pact_m1p.pdf}
\vspace{-6mm}
\caption{\textmd{\ifrmodelscaled}}
\vspace{-1mm}
\label{figures:power_2x}
    \end{subfigure}
\caption{\footnotesize{
Average power and total energy consumption.}}
%for \ifrmodel~(a) and \ifrmodelscaled(b). }}
\vspace{-4mm}

\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t!]
%\vspace{-8mm}
\begin{subfigure}{.48\columnwidth}
\includegraphics[width=1.0\textwidth, trim={0.05cm 10.0cm 18.5cm 0.05cm },clip]{Figures/power_pact_m2.pdf}
\vspace{-4mm}
\caption{\textmd{1 node \ourway} }
\vspace{-1mm}
\label{figures:power_ads}
    \end{subfigure}
\begin{subfigure}{0.48\columnwidth}
%\centering
\includegraphics[width=1.0\textwidth, trim={0.05cm 10.0cm 18.5cm 0.05cm },clip]{Figures/power_pact_m2p.pdf}
\vspace{-4mm}
\caption{\textmd{2 nodes \ourway}}
%\vspace{-1mm}
\label{figures:power_ads_2}
    \end{subfigure}
\caption{\footnotesize{
Average power and total energy consumption.}}
%for \ifrmodel~(a) and \ifrmodelscaled(b). }}
\vspace{-3mm}

\end{figure}
\begin{figure}[]
%\vspace{-8mm}
 \centering
  \includegraphics[width=0.49\textwidth, trim={0.4cm 8.3cm 10.3cm 0.05cm },clip]{Figures/endurance.pdf}
 \caption{\footnotesize{Wearout comparison for \ifrmodel~ and \ifrmodelscaled .}}
 \vspace{-2mm}
 \label{fig:endurance}
\end{figure}




\subsection{Cache hit and IO utilization}
%In this section, we show the cache hit rates and the IO resource utilization of \ifrmodel~and \ifrmodelscaled. 
Figure \ref{figures:cache_hit} shows the cache hit rates for \ifrmodel~ and \ifrmodelscaled. For \ifrmodel~ in Figure \ref{figures:cache_hit_1x }, we observe 50\% cache hit rate with \sysOne and \sysTwo that uses only DRAM for cache, and addition of \pmem~ (\sysThree) increases the cache hit to 75\%. The 768GB \pmem~ configuration (\sysFour) does not increase the cache hit further because the 384GB \pmem is enough to capture the temporal locality. As a result, both configurations of \pmem~ reach similar QPS, as shown in Figure \ref{fig:qps_ifr}. For \ifrmodelscaled, as shown in Figure \ref{figures:cache_hit_2x}, we measure 40\% cache hit rate with \sysOne. The addition of \pmem~ increases the cache hit to 60\% and 70\% for \sysThree~ and \sysFour, respectively. In this case, as shown in Figure~\ref{fig:qps_ifr_scaled}, higher \pmem~ translates to higher QPS. The reason for the different behavior by \ifrmodel~and \ifrmodelscaled~is that the bigger embedding dimension in the latter model manifests higher pressure on the caches. As a result, a larger cache size can capture more locality, resulting in less IO traffic and improved QPS. 
%Note that when we increase the model size, small size embedding tables that used to fit in HBM and DRAM are pushed to SSD. These tables fit in the cache hence, the cache hit rates stays in the same range as the \ifrmodel~  model but if we compare in terms of IO requests the 2X model still have larger IO request. 

As shown in Figure \ref{figure:iops}, the trainer achieves higher IOPS and bandwidth with \optane. In Figure \ref{figure:iops_1x} for \ifrmodel~ with \optane~ 1.5$\times$ more IOPS and 2.3$\times$ more effective BW ($IOPS \times embedding\_dim$) is measured, and consecutively more than 2$\times$ QPS compared to \flash, as shown in Figure \ref{fig:qps_ifr}. Adding \pmem decreases IOPS by up to 80\% and BW by up to 60\%. Here, the IO traffic is substantially reduced to the point that SSD traffic is not on the critical performance path. Figure \ref{figure:iops_2x} shows similar trends for \ifrmodelscaled~ with the main difference that the higher \pmem~ continues to improve QPS, and hence IOPS and effective BW. In summary, the \ourway configurations in Table \ref{tab:systems} improve QPS 1) by reducing IO traffic using \pmem or 2) by providing more IOPS using \optane.   

\begin{figure}[t!]
%\centering
\vspace{-9mm}

  \begin{subfigure}{.47\columnwidth}

%\includegraphics[width=1.15\textwidth, trim={0.01cm 8.4cm 15.2cm 0.05cm },clip]{Figures/cache_hit_m1.pdf}
\includegraphics[width=1.05\textwidth, trim={0.51cm 8.4cm 15.7cm 0.55cm },clip]{Figures/cachehit_pact_m1.pdf}
%%%\vspace{-3mm}
\vspace{-5mm}
\caption{\textmd{\ifrmodel} }
%%%\vspace{-3mm}
\label{figures:cache_hit_1x }
    \end{subfigure}
\begin{subfigure}{0.47\columnwidth}
%\centering
%\includegraphics[width=1.14\textwidth, trim={0.05cm 8.2cm 15.6cm 0.05cm },clip]{Figures/cache_hit_m1p.pdf}
\includegraphics[width=1.05\textwidth, trim={0.55cm 8.4cm 16.1cm 0.55cm },clip]{Figures/cachehit_pact_m1p.pdf}
%%%\vspace{-3mm}
\vspace{-5mm}
\caption{\textmd{\ifrmodelscaled}}
%%%\vspace{-3mm}
\label{figures:cache_hit_2x}

    \end{subfigure}
\caption{
\footnotesize{Cache hit rates for \ifrmodel (a) and \ifrmodelscaled (b) for different \ourway~ configurations.}
}
\vspace{-4mm}
\label{figures:cache_hit}
\end{figure}
%%\vspace{-3mm}

\begin{figure}[t!]
%\centering
%\vspace{-9mm}

  \begin{subfigure}{.475\columnwidth}
%\includegraphics[width=1.1\textwidth, trim={0.05cm 8.1cm 16.0cm 0.005cm },clip]{Figures/iops_m1.pdf}
\includegraphics[width=1.15\textwidth, trim={0.150cm 9.1cm 15.0cm 0.005cm },clip]{Figures/iops_pact_m1.pdf}

\vspace{-3mm}
\caption{\textmd{\ifrmodel} }
%%%\vspace{-3mm}
    \label{figure:iops_1x}
    \end{subfigure}
\begin{subfigure}{0.475\columnwidth}
%\centering
 %\includegraphics[width=0.95\textwidth, trim={0.05cm 8.1cm 18.3cm 0.05cm },clip]{Figures/iops_m1_p.pdf}
 \includegraphics[width=1.1\textwidth, trim={0.15cm 9.1cm 16.0cm 0.005cm },clip]{Figures/iops_pact_m1p.pdf}

\vspace{-3mm}
\caption{\textmd{\ifrmodelscaled}}

    \label{figure:iops_2x}
    \end{subfigure}
\caption{\footnotesize{
IOPS and effective SSD BW for \ifrmodel~and \ifrmodelscaled. }
}
\vspace{-4mm}
    \label{figure:iops}
%\vspace{-3mm}
\end{figure}




%\subsection{With and  without \ourway~}





%\begin{table}[h]
%\centering
%\footnotesize
%%%%\vspace{-3mm}

%\vspace{-8mm}
%\begin{tabular}{|l|c|c|c|c|c|}
%\hline
%& Memory cost & \ifrmodel & \ifrmodelscaled\\
%\sysOne & 1  & 1&1  \\
%\sysTwo & 1.6  & 2.15&2.75 \\
%\sysThree & 1.38  & 2.35& 1.7\\
%\sysFour & 1.77  &  2.4&2.76\\
%\sysFive & 1.98  & 2.35 &3.4\\
%Config2XDRAM & 2  & 2.7 &2.4\\
%\hline
%\end{tabular}
%%%\vspace{-4mm}
%\caption{Memory cost and QPS.}
%\label{tab:memorycost}
%\end{table}
\vspace{-2mm}
\subsection{Embedding table assignment efficiency}\label{pl}
%%\vspace{-2mm}
In this section, we compare the benefit of four embedding table placements. The first is placing all embedding tables in RocksDB storage (\flash and \optane) and using the available size of DRAM and \pmem~ memories for caching. We use this as the baseline in Figure \ref{fig:placement} and call it unoptimized because table placement is only optimized for maximizing the utilization of the sizes of SSDs instead of BW; hence, the data access volume is not balanced among the GPUs. When we compare the unoptimized with using BW to balance the data access of the GPUs, we increase QPS by 15\%. Note that using just SSD with DRAM and \pmem~ caching has lower HBM utilization. We then compare this to applying a linear programming solver with only the size of embedding tables and memory types as input. We get 2.5-3.5$\times$ more QPS with this placement. Using both size and bandwidth aware placement further increases the QPS to 3.2-4.2$\times$. Hence, table placement is critical when training DLRM with heterogeneous memories, and considering both the size and BW provides the best performance. 




%%\vspace{-2mm}









==> evaluation1.tex <==
%\vspace{-3mm}
\section{Evaluation}\label{experiments}
\subsection{Baseline}
We compare \ourway~ to the baseline system configuration shown in Table \ref{tab:systems}. Our implementation in the baseline also uses an integration of DLRM and FBGEMM\_GPU. We use HBM and DRAM in the baseline for embedding storage and caching. This implementation uses the same techniques as CDLRM \cite{balasubramanian2021cdlrm}. While CDLRM uses the CPU to manage the cache, for a fair comparison with \ourway, which uses GPU for fast cache management, we move the cache management in CDLRM to GPU. We call this CDLRM+. We also added the efficient embedding table placement in CDLRM+. Our experiments compare the number of nodes required to train a model running CDLRM+ with the performance we get with a single node running \ourway. To compare performance, we used target QPS, an acceptable QPS in our data center, to train a specific model based on the rate at which the new training data becomes available. QPS in our experiment represents the number of input data we can use to train a model per second, including the forward and backward pass. It is inversely proportional to the training time.   
\vspace{-1mm}
\subsection{Training efficiency}
One of the principal arguments for adopting denser memory technologies is to use fewer nodes for specific model training to improve power and cost-efficiency. Hence, we first compare the overall deployment efficiency of \ourway~and CDLRM+ for \ifrmodel~and \adsmodel~ based on the target QPS and the energy and power.
\begin{figure}[]
%%\vspace{-3mm}
\vspace{-10mm}

 \centering
 \includegraphics[width=0.46\textwidth, trim={0.25cm 6.8cm 5.3cm 0.05cm },clip]{Figures/qps_target_1.pdf}
 %\vspace{-2mm}
 \caption{\footnotesize{ Training QPS and number of host Comparison of CDLRM+ and \ourway~ with SLA QPS target as the baseline for \ifrmodel~ and \ifrmodelscaled }}
 \label{scale_model_1}
 \vspace{-3mm}
\end{figure}
\begin{figure}[]
%\vspace{-10mm}

 \centering
\includegraphics[width=0.47\textwidth, trim={0.25cm 7.1cm 5.3cm 0.05cm },clip]{Figures/qps_target_ads_1.pdf} 
 \caption{\footnotesize{ Training QPS and number of host Comparison of CDLRM+ and \ourway~ with SLA QPS target as the baseline for \adsmodel.}}
\vspace{-4mm}
 \label{scale_model_2}
\end{figure}
\vspace{-1mm}
\subsubsection{\textbf{Deployment efficiency}}
Figure \ref{scale_model_1} shows the efficiency comparison of \ifrmodel~and \ifrmodelscaled, which are memory capacity bound. Note that \ifrmodelscaled~ is the future scaling of \ifrmodel~ with a larger size (2$\times$). These models require 4-8 hosts to load and train with the baseline CDLRM+. With \ourway, one host can provide sufficient extended memory capacity to load and train the model. We can also reach the target QPS (SLA) in such a setting, as seen in Figure \ref{scale_model_1}. While the baseline without \ourway~ achieves higher QPS, it requires 4-8$\times$ more hosts, so this performance is stranded and does not contribute additional efficiency to the deployment because we already met our training QPS requirement. As a result, \ourway~ can improve power and cost efficiency for \ifrmodel~ and \ifrmodelscaled~ while providing SLA performance. Our experiments show that models scaled beyond \ifrmodelscaled require multi-node training, each node leveraging \ourway. Nevertheless, \ourway~ still provides a lower host count because it can store a larger model per host compared to the baseline.  

Figure \ref{scale_model_2} shows a comparison of \ourway~vs 	CDLRM+ for \adsmodel~ ( BW bound workload). This model requires 3 hosts to train with the baseline configuration. While \ourway~allows the model to be loaded and trained on one host, it does not meet QPS requirements (for both 1 node and 2 nodes running MTrainS) because of the higher memory bandwidth required by the model. However, such capability extends the efficiency of research and development without high QPS production requirements.

%In contrast, X and Y nodes are required to load the model with \pmem~or \flash~ respectively. Figure~\ref{fig:qps_ifr} shows the training QPS with different optimization and configurations. The first observation is that leveraging \optane can increase QPS by up to Z\% compared to \flash, given the lower latency and higher IOPS offered by \optane. \pmem can further increase QPS, by up to 90\% compared to \flash, by allowing bigger cache for the SSDs. 

%Given the QPS with HBM and DRAM only solution, QPS per host could be improved by G\% by avoiding the scale out. 

%We need cache hit rates, and SSD IOPS, and also discuss how much of SSD BW we are actually consuming. 
%We might need a model with a few more large features to increase BW to SSD.
%As seen in Figure \ref{scale_model_1} when we add \pmem to SSD training we achieve 1.6 - 1.85X more QPS for \ifrmodel. We can conclude that the increase in performance is due to the addition of \pmem which will increase the cache hit rate. Even when we are increasing the size of the model by 2-4X we can still accommodate for the increase in size and BW requirement. This is because of the high locality of the embedding features and with hierarchical caching, we can keep the highly accessed data in DRAM, which will provide high BW to the hot data. 




\vspace{-1mm}
\subsubsection{\textbf{Power and energy analysis}}
%%\vspace{-3mm}

 
Figure \ref{fig:baseline_energy} shows the power and energy of \ifrmodel~ and \ifrmodelscaled~ compared to the baseline configuration. Compared to training using the baseline with only HBM and DRAM, which requires 4-8 nodes to accommodate the models, we see $\sim$ 1/4 - 1/8  power reduction with \ourway. This is driven largely by the reduction in the number of nodes required. At the same time, energy is reduced by up to 55\%. However as seen in the figure, \sysOne has  higher energy than the baseline system because of the low QPS (longer training time). Note that this high reduction is because we have a QPS target for training. If we were to compare absolute performance achieved by the baseline system and \ourway, the number of nodes running \ourway required would be higher, lowering power and energy reduction.

%Figure R\ref{fig:adsbaseline_energy} shows the power and energy comparison of the baseline system with various MTrainS configurations. In the figure, we see that the average power consumption is reduced by up to 60\%  in 1 node and 30\% in 2 node MTrainS for the configurations with SCM (reduction is because of the number of nodes used compared to baseline). But when we see energy, as seen in figure 13 in the paper, the QPS for model 2 for SCM and NAND SSD training is low compared to baseline config (higher training time), hence energy consumption is very high compared to the baseline. This shows that, for bandwidth-bound workload, using storage class memories does not meet the QPS target and increases energy consumption.

Figure \ref{fig:adsbaseline_energy} shows \adsmodel's average power consumption is reduced by up to 60\% in 1 node and 30\% in 2 node \ourway configurations. However, when we see energy in Figure \ref{fig:adsbaseline_energy} because \ourway's QPS for model 2 is lower than the baseline config (longer training time), energy consumption is higher compared to the baseline. In summary, for bandwidth-bound workload, using \ourway does not meet the QPS target and increases energy consumption.

\begin{figure}[]
\vspace{-10mm}
 \centering
  \includegraphics[width=0.50\textwidth, trim={0.2cm 10.0cm 10.3cm 0.05cm },clip]{Figures/power_e_baseline.pdf}
   \vspace{-3mm}

 \caption{\footnotesize{Power and energy comparison of \ourway~ to baseline system running CLDRM+ for \ifrmodel~ and \ifrmodelscaled .}}
 \vspace{-6mm}
 \label{fig:baseline_energy}
\end{figure}
\begin{figure}[]
%\vspace{-9mm}
 \centering
  \includegraphics[width=0.50\textwidth, trim={0.2cm 9.5cm 11.3cm 0.05cm },clip]{Figures/model2_power.pdf}
  % \vspace{-3mm}

 \caption{\footnotesize{Power and energy comparison of \ourway~ to baseline system running CLDRM+ for \adsmodel~ using 1 and 2 nodes eith MTrainS.}}
 \vspace{-3mm}
 \label{fig:adsbaseline_energy}
\end{figure}

\subsection{MtrainS configs performance, energy, and power differences}

Next, we evaluate the performance of the various system configurations compared to \sysOne~ to understand the performance implication of \pmem~ and \optane~ compared to \flash. In Figure \ref{fig:qps_ifr} and \ref{fig:qps_ifr_scaled}, we compare QPS achieved for \ifrmodel~ and \ifrmodelscaled~ for different configurations of \ourway. As shown in Figure \ref{fig:qps_ifr}, for \ifrmodel, using \optane~(\sysTwo) instead of \flash~(\sysOne) increases QPS by 2$\times$. Using \pmem~with \flash~(\sysThree~ and \sysFour) increases cache size. Hence lowers traffic to \flash~ and therefore provides 2.4$\times$ QPS. Our results indicate no further improvement in QPS for the setup with both \pmem~and \optane~ for \sysFive because once we increase the cache size per host using \pmem, the access to SSDs is out of the critical path. 


%(training with \flash~ without SCM).



%For 2X size \ifrmodel, as seen in Figure \ref{fig:qps_ads}, using \flash~ with 384GB of \pmem~ increases QPS by 1.73X whereas, using 768GB of \pmem increases by 2.76X due to the increased cache hit rate. When we compare using both \pmem~ with \flash, we achieve 3.2X QPS. 2X model has much higher IO traffic than \ifrmodel~ . In this case even after we increased the cache size with \pmem~, using \optane still provides better performance because the SSD access, even though decreases using \pmem~ cache, is still in the critical path. 
\begin{figure}[t!]
%\centering
\vspace{-10mm}

  \begin{subfigure}{.50\columnwidth}

%\includegraphics[width=1.16\textwidth, trim={0.01cm 8.5cm 16.9cm 0.05cm },clip]{Figures/feed_qps_1x_1.pdf}
\includegraphics[width=1.16\textwidth, trim={0.6cm 11.5cm 16.9cm 0.05cm },clip]{Figures/model1_detail.pdf}
%%%\vspace{-3mm}
%\vspace{-5mm}
\caption{\textmd{\ifrmodel} }
%%%\vspace{-3mm}
\label{fig:qps_ifr}
    \end{subfigure}
\begin{subfigure}{0.46\columnwidth}
%\centering
%\includegraphics[width=1.15\textwidth, trim={0.05cm 8.0cm 17.02cm 0.05cm },clip]{Figures/feed_qps_2x_1.pdf}
\includegraphics[width=1.14\textwidth, trim={0.1cm 11.5cm 18.9cm 0.05cm },clip]{Figures/model1p_detail.pdf}

%%%\vspace{-3mm}
%\vspace{-5mm}
\caption{\textmd{\ifrmodelscaled}}
%%%\vspace{-3mm}
\label{fig:qps_ifr_scaled}

    \end{subfigure}
 \caption{\footnotesize{QPS comparison of different configuration of \ourway~ with \sysOne as the baseline for \ifrmodel and \ifrmodelscaled.}}
\vspace{-3mm}
%\label{figures:cache_hit}
\end{figure}



\begin{figure}[t!]
%\centering
%\vspace{-8mm}

  \begin{subfigure}{.50\columnwidth}

%\includegraphics[width=1.16\textwidth, trim={0.01cm 8.5cm 16.9cm 0.05cm },clip]{Figures/feed_qps_1x_1.pdf}
\includegraphics[width=1.21\textwidth, trim={0.5cm 11.5cm 16.5cm 0.05cm },clip]{Figures/model2_1_detail.pdf}
%%%\vspace{-3mm}
%\vspace{-5mm}
\caption{\textmd{1 Node \ourway} }
%%%\vspace{-3mm}
\label{fig:qps_ads}
    \end{subfigure}
\begin{subfigure}{0.46\columnwidth}
%\centering
%\includegraphics[width=1.15\textwidth, trim={0.05cm 8.0cm 17.02cm 0.05cm },clip]{Figures/feed_qps_2x_1.pdf}
\includegraphics[width=1.14\textwidth, trim={0.1cm 11.7cm 19.09cm 0.05cm },clip]{Figures/model2_2_detail.pdf}

%%%\vspace{-3mm}
%\vspace{-5mm}
\caption{\textmd{2 Nodes \ourway}}
%%%\vspace{-3mm}
\label{fig:qps_ads_2}

    \end{subfigure}
 \caption{\footnotesize{QPS comparison of different configuration of \ourway~ with \sysOne as the baseline for \adsmodel.}}
\vspace{-6mm}
%\label{figures:cache_hit}
\end{figure}

For \ifrmodelscaled, shown in Figure \ref{fig:qps_ifr_scaled}, \flash~with 384GB of \pmem~(\sysThree) increases QPS by 1.73$\times$ whereas, 768GB of \pmem~(\sysFour) increases by 2.76$\times$ due to the increased cache hit rate. When we use both \pmem~with \optane~(\sysFive), we achieve 3$\times$ QPS. \ifrmodelscaled~has higher BW requirement due to increased embedding dimension. With \flash~we already read 4KB blocks per IO, which is larger than the embedding dimension. Nevertheless, increased embedding dimension results in fewer embedding rows maintained in the cache (DRAM or \pmem), given fixed cache size. This increases the miss rate and hence results in increased IO to the SSDs. \optane~with higher IOPS can support such an increase in IO, hence showing higher QPS. 

In Figure \ref{fig:qps_ads} for \adsmodel with 1 node \ourway, because of \optane's higher bandwidth and lower latency compared to \flash in \sysOne, performance increases by ~2.2x. By adding \pmem we get 2x and 3.2x more performance because the cache hit increases. Similar to \ifrmodel, the combination of \pmem and \optane achieves the best performance. In figure \ref{fig:qps_ads_2}, the model is sharded between 2 nodes, and the model size per node is half of 1 node \ourway. The performance improvement for 2 nodes follows the same pattern as 1 node \ourway, but the speedup decreases compared to 1 node because SSD traffic decreases when the model size per node is reduced. Although compared to \sysOne, the various configurations show performance improvement for \adsmodel, using SCM does not provide adequate performance (QPS improvement) for memory bandwidth-bound workloads.


In Figure ~\ref{figures:power_1x} and Figure~\ref{figures:power_2x} we show the power and energy of the various \ourway~ configurations \ifrmodel~ and \ifrmodelscaled~ to study the increase in power and the total energy usage when introducing \pmem~ and \optane to our system. 
The power consumption of adding \pmem~ and \optane~ only increases the overall platform power consumption by 1-3.2\%. This is because of the low power consumption of these individual units and because major power consumption contributors are the GPU, CPU, and DRAM. This extra power consumption per node is justified when considering reduced execution time and overall Energy consumption ($Energy = Power \times Time$). We observe a 60\% to 70\% reduction in the energy consumption across the two models compared to \sysOne.

Figure \ref{figures:power_ads} and \ref{figures:power_ads_2} show the power and energy of \ourway~ for \adsmodel. In this case, adding SCMs increases the power by 18\%. This is because there are more cache and embedding storage activities in \adsmodel because it has a larger data access volume compared to \ifrmodel.





%%\vspace{-4mm}
 


% Reducing the number of hosts by 4-8 decreases training costs by approximately 4-8. To compare the implication of adding SCM, we compared the additional cost of memory in the system when introducing SCM and with equal addition of DRAM. Due to the limited DRAM in our system, we scaled down the workload size and system configuration to mimic the system with larger DRAM. Table \ref{tab:memorycost} shows a comparison of memory cost and QPS achieved. As seen in the Table, for model 1 while we meet QPS with \systemone, we can meet our endurance with \systemtwo by only adding 0.38% of the cost of total memory. For model 1+, 








%\begin{figure}[]
%\centering
% \includegraphics[width=0.5\textwidth, trim={0.05cm 9.6cm 9.3cm 0.05cm %},clip]{Figures/feed_scale.pdf}
% \caption{SSD training efficiency as we scale models for model 1 .}
% \label{scale_model_1}
%\end{figure}


\subsection{Storage endurance and wearout}
Figure \ref{fig:endurance} shows the TB written per day for \ifrmodel~ and \ifrmodelscaled~ to see if we meet our endurance requirements with the different configurations of \ourway. Based on the sizes of \optane~ and \flash, the endurances to avoid storage wear out are 200TB and 8TB data writes per day (DWPD), respectively. As seen in the figure, while we satisfy our QPS target with \sysOne~ for \ifrmodel, the write per day exceeds the endurance of \flash~(8TB). \sysTwo~ and \sysFour satisfy the endurance because of the increase in cache size and ~\sysThree~ because of the combination of cache size and BW increase in the storage. All configurations with \optane meet the endurance (200TB). For \ifrmodelscaled, all configuration backed by \flash does not meet the endurance. Hence for future models \optane~ is the best option to prevent wear out of storage.
\begin{figure}[t!]
\vspace{-10mm}
\begin{subfigure}{.48\columnwidth}
%\includegraphics[width=1.2\textwidth, trim={0.05cm 9.0cm 14.0cm 0.05cm },clip]{Figures/power_m1.pdf}
\includegraphics[width=1.3\textwidth, trim={0.05cm 9.0cm 14.5cm 0.95cm },clip]{Figures/power_pact_m1.pdf}
\vspace{-6mm}
\caption{\textmd{\ifrmodel} }
\vspace{-1mm}
\label{figures:power_1x}
    \end{subfigure}
\begin{subfigure}{0.48\columnwidth}
%\centering
%\includegraphics[width=1.0\textwidth, trim={0.05cm 8.8cm 17.5cm 0.08cm },clip]{Figures/power_m1p.pdf}
\includegraphics[width=1.0\textwidth, trim={0.05cm 8.6cm 18.9cm 0.95cm },clip]{Figures/power_pact_m1p.pdf}
\vspace{-6mm}
\caption{\textmd{\ifrmodelscaled}}
\vspace{-1mm}
\label{figures:power_2x}
    \end{subfigure}
\caption{\footnotesize{
Average power and total energy consumption.}}
%for \ifrmodel~(a) and \ifrmodelscaled(b). }}
\vspace{-4mm}

\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t!]
%\vspace{-8mm}
\begin{subfigure}{.48\columnwidth}
\includegraphics[width=1.0\textwidth, trim={0.05cm 10.0cm 18.5cm 0.05cm },clip]{Figures/power_pact_m2.pdf}
\vspace{-4mm}
\caption{\textmd{1 node \ourway} }
\vspace{-1mm}
\label{figures:power_ads}
    \end{subfigure}
\begin{subfigure}{0.48\columnwidth}
%\centering
\includegraphics[width=1.0\textwidth, trim={0.05cm 10.0cm 18.5cm 0.05cm },clip]{Figures/power_pact_m2p.pdf}
\vspace{-4mm}
\caption{\textmd{2 nodes \ourway}}
%\vspace{-1mm}
\label{figures:power_ads_2}
    \end{subfigure}
\caption{\footnotesize{
Average power and total energy consumption.}}
%for \ifrmodel~(a) and \ifrmodelscaled(b). }}
\vspace{-3mm}

\end{figure}
\begin{figure}[]
%\vspace{-8mm}
 \centering
  \includegraphics[width=0.49\textwidth, trim={0.4cm 8.3cm 10.3cm 0.05cm },clip]{Figures/endurance.pdf}
 \caption{\footnotesize{Wearout comparison for \ifrmodel~ and \ifrmodelscaled .}}
 \vspace{-2mm}
 \label{fig:endurance}
\end{figure}




\subsection{Cache hit and IO utilization}
%In this section, we show the cache hit rates and the IO resource utilization of \ifrmodel~and \ifrmodelscaled. 
Figure \ref{figures:cache_hit} shows the cache hit rates for \ifrmodel~and \ifrmodelscaled. For \ifrmodel~ in Figure \ref{figures:cache_hit_1x }, we observe 50\% cache hit rate with \sysOne that uses DRAM for cache, and addition of \pmem~ (\sysThree) increases the cache hit to 75\%. The 768GB \pmem~ configuration (\sysFour) does not increase the cache hit further because the 384GB \pmem is enough to capture the available locality. As a result, both configurations of \pmem~ reach similar QPS, as shown in Figure \ref{fig:qps_ifr}. For \ifrmodelscaled, as shown in Figure \ref{figures:cache_hit_2x}, we measure 40\% cache hit rate with \sysOne. The addition of \pmem~ increases the cache hit to 60\% and 70\% for \sysThree~ and \sysFour, respectively.  In this case, as shown in Figure~\ref{fig:qps_ifr_scaled}, higher \pmem~ translates to higher QPS. The reason for the different behavior by \ifrmodel~and \ifrmodelscaled~is that the bigger embedding dimension in the latter model manifests higher pressure on the caches. As a result, larger cache size can capture more locality, resulting in less IO traffic and improved QPS. 
%Note that when we increase the model size, small size embedding tables that used to fit in HBM and DRAM are pushed to SSD. These tables fit in the cache hence, the cache hit rates stays in the same range as the \ifrmodel~  model but if we compare in terms of IO requests the 2X model still have larger IO request. 

As shown in Figure \ref{figure:iops}, the trainer achieves higher IOPS and bandwidth with \optane. In Figure \ref{figure:iops_1x} for \ifrmodel~ with \optane~ 1.5$\times$ more IOPS and 2.3$\times$ more effective BW ($IOPS \times embedding dim$) is measured, and consecutively more than 2$\times$ QPS compared to \flash, as shown in Figure \ref{fig:qps_ifr}. With \pmem, the IO traffic is substantially reduced to the point that SSD traffic is not in the critical path of performance. Figure \ref{figure:iops_2x} shows similar trends for \ifrmodelscaled~ with the main difference that the higher \pmem~ continues to improve QPS, and hence IOPS and effective BW.   

\begin{figure}[t!]
%\centering
\vspace{-9mm}

  \begin{subfigure}{.47\columnwidth}

%\includegraphics[width=1.15\textwidth, trim={0.01cm 8.4cm 15.2cm 0.05cm },clip]{Figures/cache_hit_m1.pdf}
\includegraphics[width=1.05\textwidth, trim={0.5cm 8.4cm 15.7cm 0.55cm },clip]{Figures/cachehit_pact_m1.pdf}
%%%\vspace{-3mm}
\vspace{-5mm}
\caption{\textmd{\ifrmodel} }
%%%\vspace{-3mm}
\label{figures:cache_hit_1x }
    \end{subfigure}
\begin{subfigure}{0.47\columnwidth}
%\centering
%\includegraphics[width=1.14\textwidth, trim={0.05cm 8.2cm 15.6cm 0.05cm },clip]{Figures/cache_hit_m1p.pdf}
\includegraphics[width=1.05\textwidth, trim={0.55cm 8.4cm 16.1cm 0.55cm },clip]{Figures/cachehit_pact_m1p.pdf}
%%%\vspace{-3mm}
\vspace{-5mm}
\caption{\textmd{\ifrmodelscaled}}
%%%\vspace{-3mm}
\label{figures:cache_hit_2x}

    \end{subfigure}
\caption{
\footnotesize{Cache hit rates for \ifrmodel (a) and \ifrmodelscaled (b) for different \ourway~ configurations.}
}
\vspace{-4mm}
\label{figures:cache_hit}
\end{figure}
%%\vspace{-3mm}

\begin{figure}[t!]
%\centering
%\vspace{-9mm}

  \begin{subfigure}{.475\columnwidth}
%\includegraphics[width=1.1\textwidth, trim={0.05cm 8.1cm 16.0cm 0.005cm },clip]{Figures/iops_m1.pdf}
\includegraphics[width=1.1\textwidth, trim={0.90cm 9.1cm 15.0cm 0.005cm },clip]{Figures/iops_pact_m1.pdf}

\vspace{-3mm}
\caption{\textmd{\ifrmodel} }
%%%\vspace{-3mm}
    \label{figure:iops_1x}
    \end{subfigure}
\begin{subfigure}{0.475\columnwidth}
%\centering
 %\includegraphics[width=0.95\textwidth, trim={0.05cm 8.1cm 18.3cm 0.05cm },clip]{Figures/iops_m1_p.pdf}
 \includegraphics[width=1.05\textwidth, trim={0.95cm 9.1cm 16.0cm 0.005cm },clip]{Figures/iops_pact_m1p.pdf}

\vspace{-3mm}
\caption{\textmd{\ifrmodelscaled}}

    \label{figure:iops_2x}
    \end{subfigure}
\caption{\footnotesize{
IOPS and effective SSD BW for \ifrmodel~and \ifrmodelscaled. }
}
\vspace{-4mm}
    \label{figure:iops}
%\vspace{-3mm}
\end{figure}




%\subsection{With and  without \ourway~}





%\begin{table}[h]
%\centering
%\footnotesize
%%%%\vspace{-3mm}

%\vspace{-8mm}
%\begin{tabular}{|l|c|c|c|c|c|}
%\hline
%& Memory cost & \ifrmodel & \ifrmodelscaled\\
%\sysOne & 1  & 1&1  \\
%\sysTwo & 1.6  & 2.15&2.75 \\
%\sysThree & 1.38  & 2.35& 1.7\\
%\sysFour & 1.77  &  2.4&2.76\\
%\sysFive & 1.98  & 2.35 &3.4\\
%Config2XDRAM & 2  & 2.7 &2.4\\
%\hline
%\end{tabular}
%%%\vspace{-4mm}
%\caption{Memory cost and QPS.}
%\label{tab:memorycost}
%\end{table}
\vspace{-2mm}
\subsection{Embedding table assignment efficiency}\label{pl}
%%\vspace{-2mm}
In this section, we compare the benefit of different embedding table placements. The first is placing all embedding tables in \flash~ and using the available size of DRAM and \pmem~ memories for caching. We use this as the baseline in Figure \ref{fig:placement} and call it unoptimized because placement is not optimized for BW; hence, the data accessed is not balanced among the GPUs. When we compare the unbalanced with using BW to balance the data access of the GPUs, we increase QPS by 15\%. Note that using just SSD with DRAM and \pmem~ caching has lower HBM utilization. We then compare this to applying linear programming techniques with only the size of embedding tables and memory types as input. We get 2.5-3.5$\times$ more QPS with this placement. Using both size and bandwidth aware placement further increases the QPS to 3.2-4.2$\times$.




%%\vspace{-2mm}









==> ex.tex <==
\section{Evaluation}\label{experiments}

\subsection{Training efficiency}
 One of the main arguments for using denser memory technologies is to use less nodes for a specific model, and hence increase efficiency. This is possible for memory capacity bound models. Hence, we first compare overall deployment efficiency of \ourway vs the baseline DLRM for \ifrmodel~ and \adsmodel.

Figure \ref{scale_model_1} shows the efficiency comparison for \ifrmodel~ and \ifrmodelscaled, which is memory capacity bound. These models requires 4-8 hosts to load and train with the baseline DLRM, when only HBM and DRAM are used. With \ourway, one host can provide enough extended memory capacity to load and train the model. The target QPS can also be reached in such setting. While the baseline without \ourway~ achieves higher QPS, it requires 4-8X more hosts so this performance is stranded and does not contribute additional efficiency to the deployment. As a result, \ourway~ can improve efficiency for \ifrmodel. Our experiments show models scaled beyond 2X to estimate future workloads require multi-node training, each node leveraging \ourway. 

Figure \ref{scale_model_2} shows comparison of \ourway~ vs baseline DLRM for \adsmodel, which is bandwidth bound. This model requires 3 hosts to train with the baseline DLRM configuration without SSD. While \ourway~ allows the model to be loaded and trained on one host, it does not meet QPS requirements, given the higher memory bandwidth needed by the model. However, such capability extends the efficiency of research and development without high QPS production requirement.

%In contrast, X and Y nodes are required to load the model with \pmem~or \flash~ respectively. Figure~\ref{fig:qps_ifr} shows the training QPS with different optimization and configurations. The first observation is that leveraging \optane can increase QPS by up to Z\% compared to \flash, given the lower latency and higher IOPS offered by \optane. \pmem can further increase QPS, by up to 90\% compared to \flash, by allowing bigger cache for the SSDs. 

%Given the QPS with HBM and DRAM only solution, QPS per host could be improved by G\% by avoiding the scale out. 

%We need cache hit rates, and SSD IOPS, and also discuss how much of SSD BW we are actually consuming. 
%We might need a model with a few more large features to increase BW to SSD.
%As seen in Figure \ref{scale_model_1} when we add \pmem to SSD training we achieve 1.6 - 1.85X more QPS for \ifrmodel. We can conclude that the increase in performance is due to the addition of \pmem which will increase the cache hit rate. Even when we are increasing the size of the model by 2-4X we can still accommodate for the increase in size and BW requirement. This is because of the high locality of the embedding features and with hierarchical caching, we can keep the highly accessed data in DRAM, which will provide high BW to the hot data. 



\begin{figure}[]
 \centering
 \includegraphics[width=0.5\textwidth, trim={0.05cm 6.6cm 5.3cm 0.05cm },clip]{Figures/qps_target.pdf}
 \caption{Comparison QPS of \ourway~ with DLRM training without \ourway~ and number of platforms required for both configurations to meet target QPS.}
 \label{scale_model_1}
\end{figure}
\begin{figure}[]
 \centering
\includegraphics[width=0.5\textwidth, trim={0.05cm 6.6cm 5.3cm 0.05cm },clip]{Figures/qps_target_ads.pdf} \caption{SSD training efficiency as we scale models for model 2 .}
 \label{scale_model_2}
\end{figure}

Next, we evaluate the impact of different system configurations compared to \sysOne~with \flash~ to understand the performance implication of these memory technologies when used to accommodate model parameters. In Figure \ref{fig:qps_ifr} and \ref{fig:qps_ads}, we compare QPS achieved for \ifrmodel~ and \ifrmodelscaled. As seen in the Figures, when we compare \sysOne~, using the size and bandwidth aware embedding table assignments described in Section \ref{model assignement}, we can achieve 50\% and 66\%  better QPS. Hence, it is important to leverage the size and bandwidth characteristics of embedding tables when we have different kinds of memories. 

As shown in Figure \ref{fig:qps_ifr}, for \ifrmodel~, using \optane~(\sysTwo) instead of \flash~(\sysOne) increases QPS by 2.\ifrmodel~ . Using \pmem~ with \flash~(\sysFour) increases cache size, and hence lowers traffic to \flash~ and therefore provides 2.4X QPS. Our results indicate no further improvement in QPS for the setup with both \pmem~ and \optane~(\sysThree). This is because, for this configuration, the access to SSDs are out of the critical path once the amount of caching per host is increased using \pmem.

%For 2X size \ifrmodel, as seen in Figure \ref{fig:qps_ads}, using \flash~ with 384GB of \pmem~ increases QPS by 1.73X whereas, using 768GB of \pmem increases by 2.76X due to the increased cache hit rate. When we compare using both \pmem~ with \flash, we achieve 3.2X QPS. 2X model has much higher IO traffic than \ifrmodel~ . In this case even after we increased the cache size with \pmem~, using \optane still provides better performance because the SSD access, even though decreases using \pmem~ cache, is still in the critical path. 


For \ifrmodelscaled, as seen in Figure \ref{fig:qps_ads}, using \flash~ with 384GB of \pmem~ increases QPS by 1.73X whereas, using 768GB of \pmem~increases by 2.76X due to the increased cache hit rate. When we compare using both \pmem~ with \optane, we achieve 3.\ifrmodelscaled~ QPS. \ifrmodelscaled~ has higher BW requirement due to increased embedding dimension. With \flash~ we already read 4KB blocks per IO, which is larger than the embedding dimension. But increased embedding dimension results in less embedding rows to be captured in the cache (DRAM or \pmem), given a fix memory size. This increases the miss rate, and hence results in increased IO to the SSDs. \optane with higher IOPS can support such increase in IO, hence showing higher QPS. 


\begin{figure}[]
 \centering
   \includegraphics[width=0.45\textwidth, trim={0.4cm 11.6cm 13.3cm 0.05cm },clip]{Figures/feed_qps_1x.pdf} 
   %\caption{QPS comparison of SSD training as we add different sizes of SCM, use optane SSD and NAND SSD, and size and BW aware model assignment (NAND SSD training without caching as baseline) for model 1 .}
 \caption{QPS comparison of \ourway~ with NAND SSD and optane SSD as we add different sizes of SCM, and size and BW aware embedding table assignments (  optimized NAND SSD training without SCM cache as baseline) for model 1 .}
 \label{fig:qps_ifr}
\end{figure}

\begin{figure}[]
 \centering
  \includegraphics[width=0.45\textwidth, trim={0.4cm 11.6cm 13.3cm 0.05cm },clip]{Figures/feed_qps_2x.pdf}
 \caption{QPS comparison of SSD training as we add different sizes of SCM, and size and BW aware model assignment ( optimized SSD training without SCM cache as baseline) for model 1 .}
 \label{fig:qps_ads}
\end{figure}


